Single-Pass Object-Focused Data Selection

While unlabeled image data is often plentiful, the costs of high-quality labels pose an important practical challenge: Which images should one select for labeling to use the annotation budget for a particular target task most effectively? To address this problem, we focus on single-pass data selection, which refers to the process of selecting all data to be annotated at once before training a downstream model. Prior methods for single-pass data selection rely on image-level representations and fail to reliably outperform random selection for object detection and segmentation. We propose Object-Focused Data Selection (OFDS) which leverages object-level features from foundation models and ensures semantic coverage of all target classes. In extensive experiments across tasks and target domains, OFDS consistently outperforms random selection and all baselines. The best results for constrained annotation budgets are obtained by combining human labels from OFDS with autolabels from foundation models. Moreover, using OFDS to select the initial labeled set for active learning yields consistent improvements

==> sec/intro_old.tex <==
% \vspace{-.5cm}
\section{Introduction}
\label{sec:intro}


\begin{figure*}[h!]
    \centering
\includegraphics[width=0.99\linewidth]{sec/images/Paper2_figure1_try10.pdf}
    \caption{\textbf{Illustration of the Setup for Object-Focused Data Selection.} The figure describes our holistic setup for dealing with constrained annotation budgets for object-level prediction tasks. We first use a foundation model to generate autolabels for the entire dataset and pre-train a model using them. Subsequently, we use OFDS to select a subset of the unlabeled pool of images to be annotated by humans. The blue box in the lower left summarizes the four main steps of OFDS. Its core advancement is to use object-level features to ensure a semantic covering of the target classes through the selected objects. The subset selected by OFDS is then used to fine-tune the model.}
    \label{fig:illustration}
    % \vspace{-.5cm}
\end{figure*}
\vspace{-.1cm}
% TO DO: motivate single-pass setting. Add this: 
% Three guding principles for data selection for object-level prediction tasks: 

%     1. single-pass selection: Iterative data selection such as in active learning requires model re-training during the selection process. This setup is known to be time-consuming and can be a major bottleneck in dataset curation. Thus, we strive for a single-pass selection method, which selects the entire dataset at once. 

%     2. Model-agnostic selection: the data selection should not be specific to a single model being trained but dataset can be re-used for training different models 

%     3. Task-specific: Previous works consider data selection by specifying the annotation budget on the level of images. However, for object-level prediction tasks, the annotation budget is counted by the number of units, which are bounding boxes  

 

% Introduce OFDS which to the best of our knowledge is the first method to satisfy all these three criteria for  

The performance of machine learning systems critically depends on the availability and quality of training data \citep{zha2023data, quality_vs_quantity}. In common vision tasks such as object detection or semantic segmentation, where pixel-level annotations are required, producing high-quality labels is time-consuming and costly. Per image, labeling at pixel resolution can take between a few seconds for simple cases to over 90 minutes for complex scenes \cite{annotation_duration}. These demands make optimizing the annotation process under a limited budget a longstanding challenge in computer vision. 

Recent advances in open-world foundation models \cite{groundingDINO,groundingSAM,sam2} have opened up new annotation and data selection possibilities. These models demonstrate strong zero-shot capabilities, allowing them to generalize across tasks without further fine-tuning. However, directly deploying these large models in resource-constrained applications, such as autonomous driving, is often impractical due to their size and computational demands. In this work, we focus on training small, task-specific models and leverage foundation models to guide data selection and reduce annotation costs for object-level prediction tasks. 

Without any cost for human labeling, foundation models can provide machine generated annotations, so-called autolabels. This raises the question: \textit{Can open-world foundation models eliminate the need for pixel-level human annotations?} To investigate this, we introduce a calibration strategy for open-world object detection and segmentation models \citep{groundingDINO,sam2} to generate reliable autolabels and examine the results on different datasets \citep{pascal,cityscapes}. We find that training on the full dataset with autolabels can outperform training on human-annotated subsets in highly budget-constrained scenarios for simple tasks. However, as annotation budgets or task complexity increase, human annotations are essential.
This leads to our second question. If the quality of autolabels is not sufficient to fully replace human labels,  \textit{can foundation models be used to improve the data selection for object-level prediction tasks?} To address this question, we first need to formulate an appropriate setting for data selection. For this puropose, we introduce three criteria that a data selection method for object-level prediction tasks should fulfill in practice:

\setlist{nosep}
\begin{enumerate}[leftmargin=*,noitemsep]
    \item \textbf{Single-pass selection}: Iterative data selection, such as in active learning, requires model re-training during the selection process. This setup is known to be time-consuming and can be a major bottleneck in dataset curation. Thus, we strive for a single-pass selection method, which selects the entire dataset to be labeled at once.
    \item \textbf{Model-agnostic selection}: The data selection should not be specific to a single downstream model being trained as it should be possible to re-use it for training different models.
    \item \textbf{Task-specific selection}: Previous works on single-pass data selection specify the annotation budget on the level of images \cite{freesel,updp} without using the names of the target classes. However, for object-level prediction tasks, the annotation budget is typically charged by the number of annotated instances (for object detection) or masks (for semantic segmentation) also referred to as \textit{units}. Correctly counting the number of annotation units \textit{requires} knowledge about the target classes. Thus, knowing the class names is practically always necessary. This is unlike image classification where every images always features one label independent of the downstream task. 
\end{enumerate}

We propose object-focused data selection (OFDS) which complies with all three criteria. Our method assumes knowledge of the target class names and selects an initial subset of images from an entirely unannotated pool under the constraint of a fixed annotation budget. Unlike existing methods \cite{freesel,updp,beyond,hacon}, which rely on a fixed set of image-level feature vectors, OFDS uses foundation models to propose object-level feature vectors. This enables choosing representative objects and ensure that the selected subset semantically covers all classes, including rare ones. We illustrate data selection with OFDS in Figure \ref{fig:illustration}. 


Beyond proposing OFDS, we argue that the most effective approach to utilize a constrained annotation budget is a combination of training with autolabels and data selection. Therefore, we propose a holistic training strategy for training downstream models for object-level prediction tasks under constrained annotations budgets. First, we pre-train the downstream models on the full dataset with autolabels and then fine-tune on human-labeled subsets constrained by a fixed annotation budget. Figure \ref{fig:illustration} illustrates the training setup and shows the performance for object detection on PASCAL VOC with class imbalance. The depicted results highlight that pre-training on the autolabeled dataset combined with fine-tuning on a human-annotated subset selected through OFDS leads to the best results. \\
Our main contributions summarize as follows:
% \vspace{-.2cm}
\setlist{nosep}
\begin{enumerate}[leftmargin=*,noitemsep]
    \item \textbf{Introducing Object-Focused Data Selection (OFDS).} We present OFDS, a method that leverages object-level representations provided by foundation models to guide data selection. The core advancement of OFDS is to perform data selection with respect to semantic similarity on the level of objects rather than entire images like existing methods \cite{freesel,updp}. Curucially, OFDS performs the data selection in a single-pass manner without requiring to train any model during the data selection, and is model-agnostic and task-specific.
    \item \textbf{Empirical Demonstration of the Effectiveness of OFDS} We compare OFDS to six different baselines for single-pass data selection across three tasks and four datasets. OFDS consistently improves the performance over all existing baselines, in particular in scenarios with imbalanced class distributions.
    \item \textbf{Holistic Training Strategy for Dealing With Constrained Annotation Budgets.} We rethink training compact models for object-level downstream tasks under constrained annotation budgets by combining data selection with autolabels. Therefore, we pre-train the model on the entire dataset with autolabels and fine-tune on subsets with human labels selected through OFDS. This approach enhances performance compared to training solely with autolabels or only on human-labeled subsets as done in prior works on data selection.
    \item \textbf{Warm starting active learning.} Active learning methods commonly require a small initial labeled dataset (the ``cold start problem''). As an application, we show that using OFDS instead of a random selection for the inital data selection to ``warm start'' active learning consistently improves active learning methods for semantic segmentation and object detection.
\end{enumerate}
\vspace{-.3cm}

%-------------------------------------------------------------------------

